PrivDPR: Synthetic Graph Publishing with Deep PageRank under Differential Privacy

The objective of privacy-preserving synthetic graph publishing is to safeguard individuals' privacy while retaining the utility of original data. Most existing methods focus on graph neural networks under differential privacy (DP), and yet two fundamental problems in generating synthetic graphs remain open. First, the current research often encounters high sensitivity due to the intricate relationships between nodes in a graph. Second, DP is usually achieved through advanced composition mechanisms that tend to converge prematurely when working with a small privacy budget. In this paper, inspired by the simplicity, effectiveness, and ease of analysis of PageRank, we design PrivDPR, a novel privacy-preserving deep PageRank for graph synthesis. In particular, we achieve DP by adding noise to the gradient for a specific weight during learning. Utilizing weight normalization as a bridge, we theoretically reveal that increasing the number of layers in PrivDPR can effectively mitigate the high sensitivity and privacy budget splitting. Through formal privacy analysis, we prove that the synthetic graph generated by PrivDPR satisfies node-level DP. Experiments on real-world graph datasets show that PrivDPR preserves high data utility across multiple graph structural properties.

==> baselines.tex <==
\section{Existing Solutions}\label{Baselines}
Differential privacy has been utilized in deep learning models through DPSGD algorithms. The aim is to safeguard the privacy of training datasets. In DPSGD, the gradient $\mathbf{g}\left(x_i\right)$ is computed for each example $x_i$ in a batch $B$ of random examples. The $\ell_2$ norm of each gradient is then clipped using a threshold $C$ to control the sensitivity of $\mathbf{g}\left(x_i\right)$. The clipped gradients $\mathbf{g}\left(x_i\right)$ are summed and combined with Gaussian noise $\mathcal{N}\left(0, C^2 \sigma^2\mathbf{I}\right)$ to ensure privacy. The average of the resulting noisy accumulated gradient $\tilde{\mathbf{g}}$ is then used to update the model parameters. The expression for $\tilde{\mathbf{g}}$ is given by:
\begin{equation}\label{dpsgd_eq1}
  \tilde{\mathbf{g}} \leftarrow \frac{1}{|B|}\left(\sum_{i=1}^{|B|} \overline{\mathbf{g}}\left(x_i\right)+\mathcal{N}\left(0, C^2 \sigma^2 \mathbf{I}\right)\right).
\end{equation}

In the context of training graph-based neural network models, individual examples no longer compute their gradients independently. Instead, the features of one node can influence the gradients of other nodes in the network. For instance, in a GNN model with $K$ layers, each node has the potential to incorporate additional features from its neighbors up to $K$ hops when calculating its gradient. Considering Equation~(\ref{dpsgd_eq1}), when training GNN models, the upper bound of the sensitivity for $\sum_{i=1}^{|B|} \mathbf{\mathbf { g }}\left(x_i\right)$ becomes ${|B|} \times C$. This is because modifying one node in the graph could potentially impact all gradients in $\sum_{i=1}^{|B|} \overline{\mathbf{g}}\left(x_i\right)$. By substituting $C$ with ${|B|} \times C$ in Equation~(\ref{dpsgd_eq1}), we obtain the following equation:
\begin{equation}\label{dpsgd_eq2}
  \tilde{\mathbf{g}}^{\prime} \leftarrow \frac{1}{|B|}\left(\sum_{i=1}^{|B|} \overline{\mathbf{g}}\left(x_i\right)+\mathcal{N}\left(0, {|B|}^2 C^2 \sigma^2 \mathbf{I}\right)\right).
\end{equation}

By comparing Equation~(\ref{dpsgd_eq2}) to Equation~(\ref{dpsgd_eq1}), we observe that in order to maintain the same level of privacy protection at each step in DPSGD, the standard deviation of the Gaussian noise added to the gradients needs to be scaled up by a factor of the batch size ${|B|}$. However, this scaling can significantly affect the model's accuracy. Addressing this challenge, current research~\cite{yang2020secure,daigavane2021node,zhang2024dpar,sajadmanesh2023gap} efforts focus on reducing the high sensitivity while attaining an appropriate trade-off between privacy and utility. Furthermore, a key contributing factor to this challenge is that GNNs typically capture information within a limited hop distance in the graph. Consequently, even slight differential privacy noise can amplify the issue, ultimately restricting the GNN's ability to accurately capture complex relationships.

\textbf{Our Idea.} Unlike previous approaches, this paper diverges from the primary goal of reducing the substantial sensitivity that accompanies the achievement of node differential privacy. Instead, our approach centers around the introduction of a deep PageRank model integrated with spectral normalization. We aim to explore how even slight perturbations in the target embedding have minimal impact on the robustness of our model. By leveraging spectral normalization, we provide an alternative perspective on addressing the challenges posed by sensitivity, focusing on the model's resilience in the face of perturbations in the target embedding.
